Retroactive Parametrized Monitoring

In online monitoring, we first synthesize a monitor from a formal specification, which later runs in tandem with the system under study, incrementally receiving its progress and evolving with the system. In offline monitoring the trace is logged as the system progresses to later do post-mortem analysis after the system has finished executing. In this paper we propose retroactive dynamic parametrization, a technique that allows a monitor to revisit the past log as it progresses, while still executing in an online manner. This feature allows new monitors to be incorporated into a running system and to revisit the past for particular behaviors based on new information discovered. Retroactive parametrization also allows a monitor to lazily ignore events and revisit and process them later, when it discovers that it should have followed those events. We showcase the use of retroactive dynamic parametrization to monitor denial of service attacks on a network using network logs.

==> macros.tex <==
%\usepackage{cesar-llncs}
\NeedsTeXFormat{LaTeX2e}
\RequirePackage{cesar-llncs}[2004/1/27]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Include useful packages. %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%These are insice cesar-llncs
%\RequirePackage{amsmath}
%\RequirePackage{amssymb}
%\RequirePackage{amsthm}
%\RequirePackage{ltlfonts}
%\RequirePackage{xspace}

%for the tables
\RequirePackage{booktabs}
\RequirePackage{multirow}
\RequirePackage{dcolumn}
%for the images
\RequirePackage{graphicx}
%\RequirePackage{xspace}

%for charts
\RequirePackage{pgfplots}
\graphicspath{{figures/plots/}}
\pgfplotsset{compat=1.11}

%\newcommand{\tessla}{TeSSLa\xspace}
%\newcommand{\striver}{Striver\xspace}

\newcommand{\lola}{Lola\xspace}
\newcommand{\lolatwo}{Lola2.0\xspace}

% Feli:
\newcommand{\felitodo}[1]{\todo[linecolor=red,backgroundcolor=red!25,bordercolor=red]{Felipe: #1}}
\newcommand{\felitext}[1]{\todo[inline,linecolor=red,backgroundcolor=red!25,bordercolor=red]{Felipe: #1}}

\newenvironment{changed}{\felitodo{Review this!}\color[HTML]{a61c1c}}{\color{black}}
\newenvironment{imported}{\felitodo{Imported text:}\color[HTML]{a61c1c}}{\color{black}}
% Cesar:
\newcommand{\cesartodo}[1]{\todo[linecolor=blue,backgroundcolor=blue!25,bordercolor=blue]{Cesar: #1}}
\newcommand{\cesartext}[1]{\todo[inline,linecolor=blue,backgroundcolor=blue!25,bordercolor=blue]{Cesar: #1}}
% Martin:
\newcommand{\martintodo}[1]{\todo[linecolor=green,backgroundcolor=green!25,bordercolor=green]{Martin: {#1}}}
\newcommand{\martintext}[1]{\todo[inline,linecolor=green,backgroundcolor=green!25,bordercolor=green]{Martin: {#1}}}
% Paloma:
\newcommand{\palotodo}[1]{\todo[linecolor=violet,backgroundcolor=violet!25,bordercolor=violet]{Paloma: #1}}
\newcommand{\palotext}[1]{\todo[inline,linecolor=violet,backgroundcolor=violet!25,bordercolor=violet]{Paloma: #1}}


\newcommand{\DefOR}{\ensuremath{\hspace{0.2em}\big|\hspace{0.2em}}}
% Semantics
%
% macros for LTL fonts
%
\newcommand{\Always}{\LTLsquare}
\newcommand{\Event}{\LTLdiamond} 
\newcommand{\Next}{\LTLcircle}
\newcommand{\Prev}{\LTLcircleminus}
%\newcommand{\Until}{\LTLUntil}
\newcommand{\U}{\mathbin{\mathcal{U}}}
\newcommand{\PrevNoFirst}{\LTLcircletilde}
\newcommand{\HasAlwaysBeen}{\LTLsquareminus}
\newcommand{\Once}{\LTLdiamondminus}
\newcommand{\Since}{\mathbin{\mathcal{S}}}
\newcommand{\BackTo}{\mathbin{\mathcal{B}}}
\newcommand{\WeakPrev}{\LTLcircletilde}
\newcommand{\F}{\Event}
\newcommand{\G}{\Always}
\newcommand{\X}{\Next}
\newcommand{\SoFar}{\LTLsquareminus}
\newcommand{\Previously}{\LTLcircleminus}
\newcommand{\Before}{\LTLcircletilde}
\newcommand{\WaitFor}{\mathbin{\mathcal{W}}}

\newcommand{\reserved}[1]{\ensuremath{\mathit{#1}}\xspace}
\newcommand{\keyword}[1]{\ensuremath{\mathbf{#1}}\xspace}
\newcommand{\Syntax}[1]{\keyword{#1}}
\newcommand{\TRUE}{\keyword{true}}
\newcommand{\FALSE}{\keyword{false}}

\newcommand{\hlola}{HLola\xspace}

% syntax
\newcommand{\LOLACODE}[1]{\texttt{\footnotesize{}#1}\xspace}
\newcommand{\STRNAME}[1]{\LOLACODE{\textcolor[HTML]{eb7600}{\textbf{#1}}}}
\newcommand{\TYNAME}[1]{\LOLACODE{\textcolor[HTML]{008000}{\textbf{#1}}}}
\newcommand{\PARAMNAME}[1]{\LOLACODE{\textcolor[HTML]{96325d}{\textbf{#1}}}}
\newcommand{\frontendsize}{\footnotesize}
\newcommand{\linensize}[1]{\scriptsize{#1}}
\newcommand{\linencolor}[1]{\textcolor[HTML]{4d798f}{#1}}
\newcommand{\LOLAACC}[2]{\LOLACODE{\textbf{[}#1\textbf{|}#2\textbf{]}}}

\newcommand{\OVER}{\LOLACODE{over}}
\newcommand{\WITHINIT}{\LOLACODE{withInit}}
\newcommand{\FWDOVER}{\LOLACODE{fwdOver}}
\newcommand{\MAPOVER}{\LOLACODE{mapOver}}
\newcommand{\FWDMAPOVER}{\LOLACODE{fwdMapOver}}
\newcommand{\INPUT}{\LOLACODE{\textbf{input}}}
\newcommand{\OUTPUT}{\LOLACODE{\textbf{output}}}
\newcommand{\NOW}{\LOLACODE{\textbf{[now]}}}
\newcommand{\WHEN}{\LOLACODE{when}}
\newcommand{\UPDATING}{\LOLACODE{updating}}
\newcommand{\MOVER}{\LOLACODE{mover}}
\newcommand{\INNERNAME}[1]{\LOLACODE{\textcolor[HTML]{4d8491}{\textbf{#1}}}}
\newcommand{\IFTHENELSE}[3]{\LOLACODE{\textcolor[HTML]{1c21b8}{if} #1 \textcolor[HTML]{1c21b8}{then} #2 \textcolor[HTML]{1c21b8}{else} #3}}
\newcommand{\IFTHENELSEPH}{\IFTHENELSE{$\cdot$}{$\cdot$}{$\cdot$}}
\newcommand{\LOLASLICE}[1]{\LOLACODE{\textbf{[:}#1\textbf{]}}}


\newcommand{\LOLASPEC}[1]{\input{src/specs/autogen/lola/#1}}
\newcommand{\STRIVERSPEC}[1]{\input{src/specs/autogen/striver/#1}}

\newenvironment{qedexample}{\begin{example}}{\qed \end{example}}
\newcommand{\RETURNWHEN}[2]{\LOLACODE{\textcolor[HTML]{4d8491}{\textbf{return }}\textcolor[HTML]{eb7600}{\textbf{#1}}\textcolor[HTML]{4d8491}{\textbf{ when }}\textcolor[HTML]{eb7600}{\textbf{#2}}}}


==> src/figures/latex/macros.tex <==
\newcommand{\reserved}[1]{\ensuremath{\mathit{#1}}}
\newcommand{\LOLACODE}[1]{\texttt{#1}}
\newcommand{\STRNAME}[1]{\LOLACODE{\textcolor[HTML]{eb7600}{\textbf{#1}}}}
\newcommand{\PARAMNAME}[1]{\LOLACODE{\textcolor[HTML]{96325d}{\textbf{#1}}}}


==> src/mainidea.tex <==
\section{Ideas}
%

\subsection{Bootstrapping Online Monitors}
%
The blockchain technology provides a case in which a system is already
running, we have its history, and we cannot restart it to install a
monitor, neither can we wait for it to finish.
%
We illustrate this idea using HLola over the blockchain Tezos, but we
believe the general principle can be applied for different RV
languages and running systems.

\subsection{Online + Offline Monitoring}
%
The idea is to install new monitors while the system is already running, aka
online monitors, requiring to check the previous history, but avoiding to save
the required streams.

Guiding example: misbehaviour list.
%
Let \(A\) be a smart contract, and we want to monitor who \(A\) interacts with.
%
Assume we keep a list of misbehaving addresses, and that we can decide when an
address \(B\) is a tainted address by monitoring who \(B\) has interacted with
in the past and keep monitoring who is \(B\) interacting now.
%
In a way, we have an offline monitor that checks the past and decides if \(B\)
is a tainted address, or a good address so far, and an online monitor that
checks that \(B\) is not interacting with other tainted addresses.

On the one hand, we have that we do not know who \(B\) may be, so if we were to
monitor this property online, we would need to have the whole blockchain as a
stream, and have a set containing every tainted address.
%
On the other hand, we need information from the past to determine who is tainted
and who is not, aside from installing an online monitoring to decide who may be
a bad address.

In this sense, we need to define a mechanism enabling specification to create
and install new online monitors while also checking offline \emph{external
mechanisms}.
%
We call this external mechanisms \emph{oracles}.

